Diffusion Sampling with Momentum for Mitigating Divergence Artifacts

Despite the remarkable success of diffusion models in image generation, slow sampling remains a persistent issue. To accelerate the sampling process, prior studies have reformulated diffusion sampling as an ODE/SDE and introduced higher-order numerical methods. However, these methods often produce divergence artifacts, especially with a low number of sampling steps, which limits the achievable acceleration. In this paper, we investigate the potential causes of these artifacts and suggest that the small stability regions of these methods could be the principal cause. To address this issue, we propose two novel techniques. The first technique involves the incorporation of Heavy Ball (HB) momentum, a well-known technique for improving optimization, into existing diffusion numerical methods to expand their stability regions. We also prove that the resulting methods have first-order convergence. The second technique, called Generalized Heavy Ball (GHVB), constructs a new high-order method that offers a variable trade-off between accuracy and artifact suppression. Experimental results show that our techniques are highly effective in reducing artifacts and improving image quality, surpassing state-of-the-art diffusion solvers on both pixel-based and latent-based diffusion models for low-step sampling. Our research provides novel insights into the design of numerical methods for future diffusion work.

==> Images/DiT_images/ver1.tex <==
% \begin{figure}
%     \centering
    
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-7.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-8.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-15.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-25.pdf}

%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-6.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-7.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-8.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-15.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-25.pdf}

%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-6.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-7.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-8.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-15.pdf}
%     \includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-25.pdf}
%     \caption{Comparison of DiT images. Maybe replace with better images if possible.}
%     \label{fig:xx}
% \end{figure}

\tabulinesep=1pt
\begin{figure}
    \centering
    \begin{tabu} to \textwidth {@{}l@{\hspace{5pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{}}

        % & \noindent\parbox[c]{0.16\columnwidth}{{DPM++ \cite{}}}
        \multicolumn{1}{l}{\shortstack[l]{\scriptsize Number of steps}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize 6}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize 7}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize 8}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize 15}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize 25}}
        \\
        
        \shortstack[l]{\tiny PLMS4 \cite{liu2022pseudo}} &
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-6.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-7.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-8.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-15.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/4_0-25.pdf}} \\

        \shortstack[l]{\tiny PLMS4 w/ HB 0.9} &
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-6.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-7.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-8.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-15.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/hb/3_9-25.pdf}} \\

        \shortstack[l]{\tiny GHVB3.8} &
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-6.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-7.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-8.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-15.pdf}} & 
        \noindent\parbox[c]{0.16\columnwidth}{\includegraphics[width=0.16\textwidth]{Images/DiT_images/ghvb/3_8-25.pdf}} \\
        
    \end{tabu}
    \caption{Comparison of DiT images. Maybe replace with better images if possible.}
    \label{fig:img_dit}
\end{figure}

==> Images/artifacts_evidence/ver1.tex <==
\setlength\tabcolsep{3pt}
\begin{figure}
    \centering
    \begin{tabularx}{\textwidth}{lX}

        \shortstack[l]{\tiny (a) PLMS4 \\ \tiny 1,000 steps} & \noindent\parbox[c]{\hsize}{
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/0.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/1.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/2.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/3.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/4.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/5.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/6.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/7.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_gt/8.pdf}
        } \\ %\\[14pt]

        & \noindent\parbox[c]{\hsize}{
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/0.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/1.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/2.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/3.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/4.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/5.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/6.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/7.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_gt/8.pdf}
        } \\[15pt] % \\[16pt]

        \shortstack[l]{\tiny (a) PLMS4 \\ \tiny 10 steps} & \noindent\parbox[c]{\hsize}{
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/0.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/1.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/2.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/3.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/4.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/5.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/6.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/7.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/image_10/8.pdf}
        } \\ %\\[14pt]

        & \noindent\parbox[c]{\hsize}{
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/0.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/1.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/2.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/3.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/4.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/5.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/6.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/7.pdf}
            \includegraphics[width=0.093\columnwidth]{Images/artifacts_evidence/heatmap_10/8.pdf}
        }

        % {\tiny} & \noindent\parbox[c]{\hsize}{
        %     \foreach \x in {0,...,7} {
        %         \includegraphics[width=0.085\columnwidth]{Images/artifacts_evidence/heatmap_gt/\x.pdf}
        %         \hfill
        %     }
        %     \includegraphics[width=0.085\columnwidth]{Images/artifacts_evidence/heatmap_gt/8.pdf}
        % } \\[15pt]

        % {\tiny (b) $k = 10$} & \noindent\parbox[c]{\hsize}{
        %     \foreach \x in {0,...,7} {
        %         \includegraphics[width=0.085\columnwidth]{Images/artifacts_evidence/image_10/\x.pdf}
        %         \hfill
        %     }
        %     \includegraphics[width=0.085\columnwidth]{Images/artifacts_evidence/image_10/8.pdf}
        % } \\[12pt]

        % {\tiny} & \noindent\parbox[c]{\hsize}{
        %     \foreach \x in {0,...,7} {
        %         \includegraphics[width=0.085\columnwidth]{Images/artifacts_evidence/heatmap_10/\x.pdf}
        %         \hfill
        %     }
        %     \includegraphics[width=0.085\columnwidth]{Images/artifacts_evidence/heatmap_10/8.pdf}
        % }
    \end{tabularx}
    \caption{Comparison of generated images and their corresponding magnitudes of latent variables with and without artifacts. The latent maps are normalized and max-pooled to $16 \times 16$, with brighter colors indicating higher magnitudes. %Magnitudes are clipped to $\left[3, 10\right]$.
    }
    \label{fig:artifact_evidence}
\end{figure}

==> Images/divergence_artifacts_aba/ver1.tex <==
\begin{figure}
    \centering
    \begin{tabu} to \textwidth {
        @{}
        l@{\hspace{5pt}}
        c@{\hspace{5pt}}
        c@{\hspace{2pt}}
        c@{\hspace{5pt}}
        c@{\hspace{2pt}}
        c
        @{}
    }  
        &
        & \multicolumn{2}{c}{\scriptsize Scale before denoising}
        & \multicolumn{2}{c}{\scriptsize Scale after denoising} \\
        
        & \tiny Original ($s = 1.0$) & \tiny $s = 3.0$ & \tiny $s = 6.0$ &\tiny  $s = 3.0$ & \tiny $s = 6.0$ \\
        
        \shortstack[l]{\tiny Stable \\ \tiny Diffusion 1.5} &
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/sd15/original.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/sd15/initial_3.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/sd15/initial_6.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/sd15/final_3.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/sd15/final_6.pdf}} \\

        \shortstack[l]{\tiny Anything \\ \tiny V4.0} &
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/anythingv4/original.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/anythingv4/initial_3.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/anythingv4/initial_6.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/anythingv4/final_3.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/anythingv4/final_6.pdf}} \\

        \shortstack[l]{\tiny Pastel-mix \\ \tiny V4.0} &
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/pastel/original.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/pastel/initial_3.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/pastel/initial_6.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/pastel/final_3.pdf}} & 
        \noindent\parbox[c]{0.17\columnwidth}{\includegraphics[width=0.17\columnwidth]{Images/divergence_artifacts_aba/pastel/final_6.pdf}} \\
        
    \end{tabu}
    \caption{Comparison of samples generated from diffusion models using PLMS4 \cite{liu2022pseudo} with a guidance scale of 15 and 250 sampling steps. The initial latent code $z \in \mathbb{R}^{4 \times 64 \times 64}$ is held fixed. Multiplying a scaling factor $s$ to a specific region $A = [0, 4) \times [28, 32)^2$ after the denoising process always induces divergence artifacts in a similar area when decoding using VAE. Applying the scale factor before the denoising process leads to the occurrence of artifacts in some cases, but fundamentally changes details in images. Prompt: "A beautiful illustration of a couple looking at fireworks in a summer festival in Japan"}
    \label{fig:latent_scaling}
\end{figure}


==> Images/fig_exp.tex <==
\begin{figure}[ht]
  \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{Images/artifact_aba/SOTA_artifacts_score_2.pdf}
    \caption{ }
    \label{fig:ablation_magnitude1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{Images/artifact_aba/SOTA_artifacts_score_1.pdf}
    \caption{ }
    \label{fig:ablation_magnitude2}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{Images/damping_coeff_aba/GHVB_l2_norm.pdf}
    \caption{}
    \label{fig:ablation_on_beta}
  \end{subfigure}
  \hfill
  %\begin{subfigure}{0.19\textwidth}
  %  \includegraphics[width=\textwidth]{Images/damping_coeff_aba/GHVB_lpips.pdf}
  %  \caption{}
  %  \label{fig:ablation_on_lpips}
  %\end{subfigure}
  \hfill
  \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{Images/damping_coeff_aba/GHVB_order_of_convergence.pdf}
    \caption{}
    \label{fig:ablation_on_ghvb}
  \end{subfigure}
  \caption{(a) and (b) represent the average magnitude score, indicating the effectiveness of each method in reducing divergence artifacts. (c) shows the L2 distance in latent space between different sampling methods and the 1,000-step PLMS4 method. Adjusting $\beta$ in GHVB plays a role in interpolating between existing methods. Finally, (d) approximates the numerical order of convergence for different GHVB versions.}
  \label{fig:abalation}
\end{figure}

==> Images/highlighted_image/ver1.tex <==
% Setting for interpolation method & (1-\beta) method is identical (guidance scale, step, etc.)
% For DPM, there is no direct comparison in Interpolation Method. So, we use PLMS1.5 instead.
% DPM ; 
%   step = 20, prompt = 0, seed = 3, momentum = 0.5, guidance = 20
%   step = 20, prompt = 0, seed = 2, momentum = 0.5, guidance = 20
% PLMS4 ;
%   step = 15, prompt = 0, seed = 8, momentum = 0.5, guidance = 7.5
%   step = 15, prompt = 0, seed = 7, momentum = 0.5, guidance = 7.5
% PLMS2 (plms2_guidance25); 
%   step = 15, prompt = 0, seed = 1, momentum = 0.5, guidance = 25
%   step = 15, prompt = 0, seed = 4, momentum = 0.5, guidance = 25

% I choose momentum (beta) = 0.5 (i.e. the midpoint) to demonstrate performance in the most stupid case. We can tune \beta to further increase image quality. Maybe we can include that in the Appendix.

% maybe consider add number of steps near the scheduler name at the top to save space?
\tabulinesep=1pt
\begin{figure}
    \centering
    \begin{tabu} to \textwidth {@{}l@{\hspace{5pt}}c@{\hspace{2pt}}c@{\hspace{4pt}}c@{\hspace{2pt}}c@{\hspace{4pt}}c@{\hspace{2pt}}c@{}}
        % & \noindent\parbox[c]{0.14\columnwidth}{{DPM++ \cite{}}} 
        & \multicolumn{2}{c}{\shortstack{\scriptsize DPM-Solver++ \cite{lu2022dpm} \\ \scriptsize Guidance scale = 20, Step = 20}}
        & \multicolumn{2}{c}{\shortstack{\scriptsize PLMS2 \cite{liu2022pseudo} \\ \scriptsize Guidance scale = 25, Step = 15}}
        & \multicolumn{2}{c}{\shortstack{\scriptsize PLMS4 \cite{liu2022pseudo} \\ \scriptsize Guidance scale = 7.5, Step = 15}} \\
        
        \shortstack[l]{\tiny Without \\ \tiny Momentum} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/original/dpm.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/original/dpm-2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/original/plms2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/original/plms2-2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/original/plms4.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/original/plms4-2.pdf}} \\

        \shortstack[l]{\tiny With \\ \tiny HB 0.5} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/interpolation_method/dpm.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/interpolation_method/dpm-2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/interpolation_method/plms2.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/interpolation_method/plms2-2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/interpolation_method/plms4.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/interpolation_method/plms4-2.pdf}} \\

        \shortstack[l]{\tiny GHVB with \\ \tiny Momentum 0.5} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/one-minus-beta_method/dpm.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/one-minus-beta_method/dpm-2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/one-minus-beta_method/plms2.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/one-minus-beta_method/plms2-2.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/one-minus-beta_method/plms4.pdf}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/highlighted_image/one-minus-beta_method/plms4-2.pdf}}
    \end{tabu}
    \caption{Comparison between samples from well-known schedulers using different methods. Using Momentum significantly reduces artifacts. Prompt: "a girl face in modern Disney style".}
    \label{fig:highlighted_image}
\end{figure}

==> Images/main_fig/00fig.tex <==
\begin{figure}
    \centering
    \begin{tabu} to \textwidth {@{}l@{\hspace{5pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{5pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{}}  
        & \multicolumn{3}{c}{\scriptsize DPM-Solver++ (2M) \cite{lu2022dpm}}
        & \multicolumn{3}{c}{\scriptsize PLMS4 \cite{liu2022pseudo}} \\
        
        & \tiny (a) & \tiny (b) &  \tiny (c) &\tiny  (a) & \tiny (b) & \tiny (c) \\
        
        \shortstack[c]{\tiny Without \\ \tiny Momentum} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_1_1.png}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_1_2.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_1_3.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_1_4.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_1_5.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_1_6.png}} \\

        \shortstack[c]{\tiny With \tiny HB 0.5 \\ \tiny (Ours)} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_2_1.png}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_2_2.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_2_3.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_2_4.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_2_5.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_2_6.png}} \\

        \shortstack[c]{\tiny GHVB 1.5 \\ \tiny (Ours)} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_3_1.png}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_3_2.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_3_3.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_3_4.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_3_5.png}} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/main_fig/1_3_6.png}} \\
        
        & \tiny $s = 15$ & \tiny $s = 25$ &  \tiny $s = 20$ &\tiny  $s = 8$ & \tiny $s = 6$ & \tiny $s = 6$ 
    \end{tabu}
    \caption{Demo }
    \label{fig:highlighted_image2}
\end{figure}

==> Images/motivate_GHVB/ver1.tex <==
% guidance scale = 15, seed = 46, steps = 15, 
\tabulinesep=1pt
\begin{figure}[ht]
    \centering
    \begin{tabu} to \textwidth {
        @{}
        l@{\hspace{6pt}}
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
        c@{\hspace{2pt}}
        c@{}
        c@{\hspace{10pt}} | @{\hspace{5pt}}
        c
        @{}
    }
        % & \noindent\parbox[c]{0.14\columnwidth}{{DPM++ \cite{}}} 
        % & \multicolumn{4}{c}{\shortstack{\scriptsize DDIM \cite{} \\ \scriptsize 1000 steps}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.2$}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.4$}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.6$}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.8$}} &
        & \multicolumn{1}{c}{\shortstack{\tiny PLMS4 $(\beta = 1.0)$}} \\

        \shortstack[l]{\scriptsize (a) PLMS4 with HB} &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/HB/3_2.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/HB/3_4.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/HB/3_6.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/HB/3_8.pdf}} & &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/PLMS4.pdf}} \\

        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.2$}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.4$}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.6$}}
        & \multicolumn{1}{c}{\shortstack{\scriptsize $\beta = 0.8$}} &
        & \multicolumn{1}{c}{\shortstack{\tiny DDIM \cite{song2020denoising}, 1000 steps}} \\

        \shortstack[l]{\scriptsize (b) 4th order GHVB } &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/GHVB/3_2.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/GHVB/3_4.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/GHVB/3_6.pdf}} & 
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/GHVB/3_8.pdf}} & &
        \noindent\parbox[c]{0.14\columnwidth}{\includegraphics[width=0.14\columnwidth]{Images/motivate_GHVB/ddim.pdf}}

    \end{tabu}
    \caption{The image shows a comparison of two momentum-based techniques, HB (a) and GHVB (b), used to reduce artifacts in PLMS4 \cite{liu2022pseudo} with 15 sampling steps. Both techniques are effective in reducing artifacts, but the accuracy of HB drops faster than GHVB. The disappearance of the tree in (a) is visible when choosing $\beta \leq 0.4$, as (a) has a lower order of convergence than (b). Prompt: "A beautiful illustration of people releasing lanterns near a river".}
    \label{fig:motivate_GHVB}
\end{figure}

==> content/bin/5_4Ablation.tex <==
\subsection{Ablation Study of GHVB} \label{sec:exp_ghvb}
\begin{minipage}{0.62\textwidth}
In this section, we conduct an ablation study of the GHVB method. As explained in Section \ref{sec:ghvb}, the damping coefficient $\beta$ of GHVB interpolates between two existing AB methods, DDIM and PLMS2. Our goal here is to analyze the convergence error of GHVB methods. The comparison is done on Stable Diffusion 1.5 with the target results obtained from a 1,000-step PLMS4 method. We measure the mean L2 distance between the sampled results and the target results in the latent space. The results in Figure \ref{fig:ablation_on_beta} suggest that the convergence error of GHVB 1.1 to GHVB 1.9 interpolates between the convergence errors of DDIM and PLMS2 accordingly.

%\end{minipage}
%\hspace{0.01\textwidth}
%\begin{minipage}{0.34\textwidth}


%\centering


%\end{minipage}


%\begin{minipage}{0.65\textwidth}
Furthermore, we empirically verify that GHVB does achieve high order of convergence as predicted by Theorem \ref{thm:ghvb}.
%GHVB is a new method, and it is crucial to verify its ability to achieve the high order of convergence predicted by Theorem \ref{thm:ghvb}. 
We compute the numerical order of convergence using the formula $q \approx \frac{\log(e_{\text{new}} / e_{\text{old}})}{\log(k_{\text{new}} / k_{\text{old}})}$, where $e$ is the error between the sampled and the target latent codes, and $k$ is the number of sampling steps. As shown in Figure \ref{fig:ablation_on_ghvb}, the numerical orders of GHVB 0.5 and GHVB 1.5 approach 0.5 and 1.5, respectively, as the number of steps increases. However, for GHVB 2.5 and GHVB 3.5, the estimated error $e$ may be too small when tested with large numbers of steps, and other sources of error may hinder their convergence. 
Nonetheless, these GHVB methods can achieve high orders of convergence. A detailed analysis of this and other methods is in Appendix \ref{apx:order}.

\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}{0.37\textwidth}
\centering

    \includegraphics[width=.99\textwidth]{Images/damping_coeff_aba/GHVB_l2_norm.pdf}
\vspace{-0.13\textwidth}
\captionsetup{type=figure}
\caption{L2 distance in latent space between different sampling methods and the 1,000-step PLMS4 method.}
\label{fig:ablation_on_beta}

\includegraphics[width=0.99\textwidth]{Images/damping_coeff_aba/GHVB_order_of_convergence.pdf}
\vspace{-0.13\textwidth}
\captionsetup{type=figure}
\caption{the numerical order of convergence for GHVB.}
\label{fig:ablation_on_ghvb}
\end{minipage}

==> content/bin/old_content.tex <==
\section{Submission of papers to NeurIPS 2023}


Please read the instructions below carefully and follow them faithfully. \textbf{Important:} This year the checklist will be submitted separately from the main paper in OpenReview, please review it well ahead of the submission deadline: \url{https://neurips.cc/public/guides/PaperChecklist}.


\subsection{Style}


Papers to be submitted to NeurIPS 2023 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2023 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2023.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2023 is \verb+neurips_2023.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS. 


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2023.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2023+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2023}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2023/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}



\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}


\section{Supplementary Material}

Authors may wish to optionally include extra information (complete proofs, additional experiments and plots) in the appendix. All such materials should be part of the supplemental material (submitted separately) and should NOT be included in the main submission.


==> tables/confidence_convergence_ghvb_lpips.tex <==
\begin{table}
\centering
\small
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{7}{c}{Number of steps}                                                                    \\
 Method & 10           & 20           & 40           & 80           & 160          & 320          & 640          \\ \hline
DDIM                 & 0.354 $\pm$ .010 & 0.287 $\pm$ .011 & 0.229 $\pm$ .013 & 0.174 $\pm$ .013 & 0.128 $\pm$ .013 & 0.089 $\pm$ .010 & 0.058 $\pm$ .008 \\
GHVB1.1              & 0.354 $\pm$ .010 & 0.283 $\pm$ .011 & 0.220 $\pm$ .013 & 0.159 $\pm$ .013 & 0.107 $\pm$ .012 & 0.062 $\pm$ .008 & 0.027 $\pm$ .005 \\
GHVB1.3              & 0.356 $\pm$ .011 & 0.282 $\pm$ .011 & 0.209 $\pm$ .013 & 0.140 $\pm$ .013 & 0.086 $\pm$ .011 & 0.038 $\pm$ .006 & 0.015 $\pm$ .004 \\
GHVB1.5              & 0.359 $\pm$ .011 & 0.278 $\pm$ .011 & 0.200 $\pm$ .014 & 0.129 $\pm$ .013 & 0.072 $\pm$ .010 & 0.028 $\pm$ .005 & 0.011 $\pm$ .003 \\
GHVB1.7              & 0.364 $\pm$ .011 & 0.279 $\pm$ .012 & 0.196 $\pm$ .014 & 0.120 $\pm$ .013 & 0.060 $\pm$ .009 & 0.023 $\pm$ .005 & 0.008 $\pm$ .002 \\
GHVB1.9              & 0.369 $\pm$ .012 & 0.281 $\pm$ .012 & 0.191 $\pm$ .014 & 0.112 $\pm$ .013 & 0.051 $\pm$ .008 & 0.019 $\pm$ .004 & 0.006 $\pm$ .002 \\
PLMS2                & 0.373 $\pm$ .012 & 0.282 $\pm$ .012 & 0.191 $\pm$ .014 & 0.110 $\pm$ .012 & 0.049 $\pm$ .007 & 0.017 $\pm$ .004 & 0.005 $\pm$ .002 \\ \hline
\end{tabular}
\caption{95\% confidence interval for LPIPS norm in GHVB (similar to figure 8c, just in case)}
\end{table}
